EXCGEC: A Benchmark for Edit-Wise Explainable Chinese Grammatical Error Correction

Existing studies explore the explainability of Grammatical Error Correction (GEC) in a limited scenario, where they ignore the interaction between corrections and explanations and have not established a corresponding comprehensive benchmark. To bridge the gap, this paper first introduces the task of EXplainable GEC (EXGEC), which focuses on the integral role of correction and explanation tasks. To facilitate the task, we propose EXCGEC, a tailored benchmark for Chinese EXGEC consisting of 8,216 explanation-augmented samples featuring the design of hybrid edit-wise explanations. We then benchmark several series of LLMs in multi-task learning settings, including post-explaining and pre-explaining. To promote the development of the task, we also build a comprehensive evaluation suite by leveraging existing automatic metrics and conducting human evaluation experiments to demonstrate the human consistency of the automatic metrics for free-text explanations. Our experiments reveal the effectiveness of evaluating free-text explanations using traditional metrics like METEOR and ROUGE, and the inferior performance of multi-task models compared to the pipeline solution, indicating its challenges to establish positive effects in learning both tasks.

==> chapters/checklist.tex <==
\section{Reproducibility Checklist}


\paragraph{This paper:}

\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced. Yes.

    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results. Yes.

    \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper. Yes.
    
\end{itemize}

\paragraph{Does this paper make theoretical contributions?} No.

\paragraph{Does this paper rely on one or more datasets?} Yes.

\begin{itemize}
    \item A motivation is given for why the experiments are conducted on the selected datasets. Yes.

    \item All novel datasets introduced in this paper are included in a data appendix. Partial.

    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. Yes.
    
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. Yes.
    
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. Yes.
    
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. Yes.

\end{itemize}


\paragraph{Does this paper include computational experiments? (yes/no)} Yes.

\begin{itemize}
    \item Any code required for pre-processing data is included in the appendix. No, but we will publicize all the codes after the review period.
    
    \item All source code required for conducting and analyzing the experiments is included in a code appendix. No, but we will publicize all the codes after the review period.
    
    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. Yes.
    
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from. Yes.
    
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. Yes.
    
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. Partial.
    
    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. Yes.
    
    \item This paper states the number of algorithm runs used to compute each reported result. Yes.
    
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. No.
    
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). No.
    
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. Yes.
    
    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. Yes.

\end{itemize}
